Capturing Smart Contract Design with DCR Graphs

Smart contracts manage blockchain assets and embody business processes. However, mainstream smart contract programming languages such as Solidity lack explicit notions of roles, action dependencies, and time. Instead, these concepts are implemented in program code. This makes it very hard to design and analyze smart contracts. We argue that DCR graphs are a suitable formalization tool for smart contracts because they explicitly and visually capture the mentioned features. We utilize this expressiveness to show that many common high-level design patterns representing the underlying business processes in smart contract applications can be naturally modeled this way. Applying these patterns shows that DCR graphs facilitate the development and analysis of correct and reliable smart contracts by providing a clear and easy-to-understand specification.

==> components/SC-semantics-to-dcr.tex <==
\subsection{Smart Contract Semantics in DCR Graphs}\label{sec:semantics2dcr}
\subsubsection{Constructor Event}
While modeling using DCR graphs, constructor can be used as the entry point to including all the activities that are available after contract deployment. This entry point becomes especially important when initialization related to access control and time-constrained activities are required at contract deployment. Furthermore, as in figure \ref{fig:constructor-activity} this initialization event is useful for including certain activities based on exact value of initialized variables.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/constructor-activity.pdf}
    \caption{Modeling specific events that are initiated once smart contract is being deployed.}
    \label{fig:constructor-activity}
\end{figure}


\subsubsection{Conditional Function Calls}
A transaction calling a contract function can trigger multiple consecutive calls conditionally. The conditional part is easily modeled by using a guard on the logical inclusion/exclusion arrows in DCR (figure \ref{fig:conditional-calls}).

\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/conditional-function-calls.pdf}
    \caption{Modeling simple conditional function calls in DCR graphs}
    \label{fig:conditional-calls}
\end{figure}


\subsubsection{Conjunction and Disjunction Operators}
These modeled operators are useful for the cases where feasibility of one action is limited to when two or more events happen in conjunction or disjunction. An example of this type of model is provided in figure \ref{fig:conjdis}.

\begin{figure}[H]
    \centering
    \includegraphics[width=1\textwidth]{figures/conj-dis.pdf}
    \caption{Disjunction (left) and conjunction (right) modeled for function calls. }
    \label{fig:conjdis}
\end{figure}


\subsubsection{Transactions in Ethereum}
% topic: what blockchain transactions really are (official definition);
Etheruem is by definition a transactional state-machine where successful transactions alter the state of distributed ledger \cite{EthereumYellowPaper2022}. Since Ethereum is a transaction-based system, atomic transactions might be expected. However, atomic transactions are not part of Ethereum transaction semantics \cite{makescsmarter}. Lack of atomicity property is the direct result of exception handling mechanisms in Solidity language. Existence of EVM opcodes such as CALL, CALLCODE, DELEGATECALL, and STATICCALL enables contract code to invoke code from another contract address amidst its execution \cite{EthereumYellowPaper2022}. These types of calls are referred to as \textit{external contract calls} in solidity. This feature also enables the contract code to handle exceptions as a result of external calls. As a result, during the original transaction even when an exception happens, it can be suppressed by the caller. In other words, part of the issued transaction code fails and another part succeeds which violates atomicity of transactions.\\
Modeling the smart contract behavior via DCR graphs in a high-level hides the complexities regarding mentioned transaction details. However, there exist situations where the behavior of each transaction is also necessary to specify. This of course leaves the specification built by DCR graphs dependent on the specific blockchain platform (here, Ethereum), and the model loses its generality.\\
Details of transactions can be modeled by using the \textit{subgraph} in DCR graphs. Before a subgraph and the acitvities it groups are available to execute, it should be spawned by another activity. In the example in figure \ref{fig:transaction-concept}, the execution of \textit{participate} will spawn \textit{vote}. It is possible to spawn multiple subgraphs of the same \textit{vote} by continuously executing \textit{participate}. The execution and termination of each of these subgraphs will be independent from each other.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/transaction-concept.pdf}
    \caption{A transaction model using subgraphs}
    \label{fig:transaction-concept}
\end{figure}

Sometimes the same function call in Ethereum is processed through different paths depending on the storage variables and state of blockchain in different transactions. The \textit{voteProposal} in \textit{Bridge.sol} \cite{Chainbridgesolidity2022a} is such a function. These different execution paths can be modeled as different entry points for the same function in different transactions. Modeling a transaction and not setting a strict order between activities in its subgraphs models the same concept. In figure \ref{fig:tx-concept-2}, most of the activities in the subgraph are included by default. Execution of each of them will affect the availability of the other acitivites and fate of the transaction. Furthermore, there is no strict order between \textit{Authorize} and \textit{Nuclear code} activities.


\begin{figure}[H]
    \centering
    \includegraphics[width=1\textwidth]{figures/startAwGame.pdf}
    \caption{Example contract modeling multiple execution paths of the same function in different transactions}
    \label{fig:tx-concept-2}
\end{figure}

\subsubsection{Block Number}
Sometimes success of a transaction depends on a condition on block number or other related concepts such as time (concept of time is retrieved from block timestamp in Ethereum). To incorporate such conditional executions in the model we can have an activity which executes and its value increases on fixed intervals independently from other components of the model. Since block number is one of the only sources of monotonically increasing value by time, modeling it to incorporate in the behavioral model of the contracts is important. Here, we construct such a model using reflexive pending arrow with a deadline on a computational activity with integer type in figure \ref{fig:blockNumber}. The role assigned to this activity is \textit{Ethereum}, and to correctly simulate its function one should simulate this role with automatic aggressive agent in DCR portal. The default pending (exclamation mark) on the activity forces the aggressive agent to execute it within the bounds of the specified deadline. At each execution the integer value of \textit{blockNumber} activity will be increased by one. Furthermore, after each execution (here every one second), a new pending deadline is registered for the activity.Figure \ref{fig:blockNumber-swimlane} shows an example simulation of the model according to the mentioned configurations in DCR portal where \textit{blockNumber} is executed at a fixed interval.
\begin{figure}[H]
    \centering
    \includegraphics{figures/blockNumber.pdf}
    \caption{Modeling block number automatic increment in DCR graphs.}
    \label{fig:blockNumber}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/blockNumber-swimlane.pdf}
    \caption{Swimlane of the blockNumber increasing every second generated during the simulation.}
    \label{fig:blockNumber-swimlane}
\end{figure}



==> components/analysis.tex <==
\section{Analysis}\label{sec:analysis}

\subsection{Application: Runtime Monitoring (CLawK)}\label{sec:clawk}
To show a simple use case of the DCR model of smart contracts, we developed a runtime monitoring tool that enables the DCR model to be simulated alongside the execution of the implementation on Ethereum networks. Figure \ref{fig:clawksystemmodel} shows the system architecture of our tool CLawK (Contract Law Keeper). The monitoring tool has three components: DCR graph execution engine, monitor backend, and GUI web interface. DCR engine executes the model in parallel to the execution of the deployed contract on Ethereum. Each time a transaction of the desired contract is initiated, the transaction details are extracted, translated to an activity in the DCR model, and sent to the DCR model simulation engine by the monitor backend. \\
The monitor backend can then detect if there is a violation in the step sent to the DCR engine based on the DCR engine API response for that step. The simulation will either continue to the next step or fall behind the deployed contract execution, which shows the contract behavior violates the model's behavior. \\
Compared to other runtime verification tools such as ContractLarva \cite{rvethereum}, CLawK currently neither supports automatic verification of properties nor automatic code patching after detecting a violation. However, using CLawK for high-level properties such as the order of activities and access control over activities does not require any contract code instrumentation. 

\begin{figure}[H]
    \centering
    \includegraphics[width=1\textwidth]{figures/monitor-system-arch.pdf}
    \caption{CLawK system model. CLawK uses the DCR graphs execution engine to monitor the runtime execution of deployed contracts on Ethereum.}
    \label{fig:clawksystemmodel}
\end{figure}


Figure \ref{fig:clawkinaction} shows a simple usage of the CLawK graphical interface in conjunction with a sample contract which only has two functions that should be executed strictly in a specific order. In the example \ref{fig:clawkinaction}, making a transaction to the wrong function first triggers an alarm since the corresponding model simulation step does not accept the target function of the transaction. Conversely, the second and third transactions are in the correct order and do not raise the alarm in the tool interface. 

\begin{figure}[H]
    \centering
    \includegraphics[width=1\textwidth]{figures/clawk-in-action.pdf}
    \caption{Using CLawK to monitor the order of actions during runtime.}
    \label{fig:clawkinaction}
\end{figure}


\subsection{Conformance Testing of Upgrades}
Contract code is an immutable part of it that is deployed only once. However, using a proxy pattern where a contract (often the proxy itself) holds the storage, and one holds the logic is possible in practice. In a simple scenario, the proxy has to delegate any call with the original \textit{calldata} to the logic contract. The address of the logic contract in the proxy can be replaced with the upgraded one. \\
Delegating a call to the logic contract gives it full access to the data-holding contract. It can significantly endanger funds and other participating user data if the behavior is not strictly as expected. This is where modeling the original logic contract using DCR graphs and testing the contract for conformance with the model during the runtime can reduce the risks akin to high-level properties of roles, access control, and partial ordering of function executions. As depicted in figure \ref{fig:upgrade-with-dcr} it is feasible to use the DCR model of the original contract both as a visual specification to develop the upgraded version and as a runtime monitor with the help of CLawK (section \ref{sec:clawk}).

\begin{figure}[H]
    \centering
    \includegraphics[width=0.6\textwidth]{figures/upgradibility-with-dcr.pdf}
    \caption{Applciation of DCR graphs in building smart contracts conforming to the original high-level specifications.}
    \label{fig:upgrade-with-dcr}
\end{figure}



%\section{Application: Automatic Contract Generation }
%We can transpile from DCR to Solidity to generate smart contract skeletons that preserve high-level properties. 



==> components/dcr.tex <==



\begin{definition}
%[\!\!\!\protect{\cite[Def.~3.2]{DCRtime}}]
\label{def:timedDCR}
    A \emph{timed DCR graph with data} $G$ is given by a tuple 
    $(E,  D, M, \conditionrel, $ $ \responserel, \noresponserel, \milestonerel, \includerel, \excluderel, L,l)$
    where 
    \begin{enumerate}%[label=(\roman*)]
    \item $E$ is a finite set of \emph{events}, 
  %\item $V:E\rightharpoondown \VAL$ is the \emph{value function}
 \item $D:E\rightarrow \mathsf{Exp_E}\uplus\{?\}$ is the \emph{data function}
    \item  $M = (\Ex,\Re,\In,\Va) \in  \bigl(
        {(E\rightharpoondown \omega)
        \mathrel\times
        {(E\rightharpoondown\infty)}
        \times
        \mathcal{P}_f(E)
        \times (E\rightharpoondown \VAL)}
        \bigr)$ 
    is the \emph{timed marking with data}, 
     \item $\conditionrel \subseteq E \times \omega \times \mathsf{BExp_E} \times E$, is the \emph{guarded timed condition relation}, 
     \item $\responserel \subseteq E \times \infty \times \mathsf{BExp_E} \times E$, is the guarded timed response relation,
    \item $\noresponserel,\milestonerel,\includerel,\excluderel\subseteq E \times \mathsf{BExp_E} \times E$ are the guarded cancel, milestone, include and exclude relations respectively,
    \item $L$ is the set of labels,
    \item $l\colon E \to L$ is a labeling function between events and labels.
    \end{enumerate}
   %We require that the data expression of an event respect the type %of events, i.e. if $D(e)\in \mathsf{BExp_E}$ then %$T(e)=\mathsf{Bool}$, if $D(e)\in \mathsf{IExp_E}$ then %$T(e)=\mathsf{Int}$, if $D(e)\in \mathsf{SExp_E}$ then %$T(e)=\mathsf{String}$ and if $D(e)=\mathsf{void}$ then %$T(e)=\mathsf{Void}$. 
   If $D(e)=~?$, we say that the event is an \emph{input event}; otherwise, it is a \emph{computation event}.
   %$T(e)\in \{\mathsf{Int},\mathsf{Bool},\mathsf{String}\}$ 
   %and its data value is provided by the environment when the event is %executed. 
   The marking $M = (\Ex,\Re,\In,\Va)$ consists of three functions and a set of events, which define the state of the process. The function $\Ex$ records each event's time since it was last \emph{{\bf Ex}ecuted}. The function $\Re$ records the deadline for when a \emph{pending {\bf Re}sponse} event is required to happen (if it is included). The set $\In$ records the currently {{\bf In}cluded events}. Finally, the \emph{{\bf Va}lue function} $\Va:E\rightharpoondown \VAL$ assigns the current value of an event if defined. We require that if $Ex(e)$ is defined, then $\Va(e)$ is defined.
   %We will write $e\in \In$ for $\In(e)=\top$, and in this case say that the event $e$ is included in %the marking.
   %We require that the marking respect the type of events, i.e. if %$Ex(e)=(n,b)$ then $T(e)=\mathsf{Bool}$, if $Ex(e)=(n,z)$ then %$T(e)=\mathsf{Int}$, if $Ex(e)=(n,z)$ then $T(e)=\mathsf{String}$ %and if $Ex(e)=(n,\bot)$ then $T(e)=\mathsf{Void}$. 
   For $d\in \mathsf{Exp_E}$ let $\evalexp{d}{M}$ be the %inductively %defined 
   evaluation relation on events relative to the marking $M$. 
   %where $\evalexp{e}{M}=v$ if $Ex(e)=(n,v)$ and defined in the %obvious way for the rest of the cases.
\end{definition}


==> components/discussion.tex <==
\section{Discussion}
\begin{table}[H]
\caption{Source code properties vs DCR graph properties for modeled contracts }
\centering
% the total length should add up to 12cm
\begin{threeparttable}
{\footnotesize
\begin{tabular}{ |p{2.7cm}||p{0.8 cm}|p{1cm}|p{2.5cm}| p{2.5cm}|p{0.7cm}|p{0.7cm}| }
\hline
\textbf{Contract}  & \textbf{LOC} & \textbf{Deps}\tnote{1} & \textbf{DCR acitivities} & \textbf{DCR arrows} & \textbf{F}\tnote{2} & \textbf{PF}\tnote{3}\\

\hline
Chainsafe Bridge & 505    & 7 & 12 & 19 & 28 & 18\\
\hline
Access Control & 247    & 4 & 3 & 2 & 12 & 7 \\
\hline
Casino & 193    & 0 & 8 & 19 & 10 & 10\\
\hline
English Auction & 85    & 1 & 5 & 8 & 4 & 4\\
\hline
Escrow & 76    & 0 & 5 & 4 & 3 & 3\\
\hline
BirthdayGift & 56    & 0 & 5 & 8 & 2 & 2\\
\hline
\end{tabular}


\begin{tablenotes}
\item[1] Contract dependencies including inheritance and external calls through external contract interface
\item[2] Total number of functions
\item[3] Total number of non-view functions 

\end{tablenotes}

}
\end{threeparttable}
\end{table}


\subsection{Shortcomings}
\todo[inline]{Discuss these in the meeting:}
\begin{enumerate}
    \item There is no explicit way to model function parameters in this modeling. Function parameters can only be modeled by using activities nested in the function activity.
    \item There is no way to initialize an activity that has a type such as integer. 
\end{enumerate}
There is no efficient way to model function parameters in this modeling.








\begin{comment}
\begin{table}[H]
\caption{Applicability of DCR modeling for Solidity-specific design patterns}
\centering
% the total length should add up to 12cm

\begin{threeparttable}
{\footnotesize
\begin{tabular}{ |p{3cm}|p{3cm}|}
\hline
Applicable\tnote{1} & Inapplicable\tnote{2} \\
\hline
 15 & 2  \\
\hline
\end{tabular}


\begin{tablenotes}
\item[1] Modeled in this work or possible to model using a combination of techniques introduced here.
\item[2] Not possible due to current limitations of DCR semantics
\end{tablenotes}

}

\end{threeparttable}
\end{table}
\end{comment}









\subsection{Effectiveness Requirements}
% what are some of the properties of the smart contracts we would like to model/monitor? 1. order of activities is important 2. there is a notion of roles and role-based access control. 

\todo{Talk about the lack of transitioning from one role to another role when a particular activity is executed, and that this feature is gonna be added (?)}
\todo{Does DCR modeling help for attack modeling in any way? https://composable-security.com/blog/threat-modeling-for-smart-contracts-best-step-by-step-guide/}




==> components/learnt-lessons.tex <==
\section{Lessons Learnt Modeling Implemented Contracts}\label{sec:learnt}
\subsection{Entangled access controls}
\textit{adminAddRelayer} function (listing \ref{lst:adminAddRelayer}) from bridge contract \cite{Chainbridgesolidity2022a} does not explicitly check for admin permission. Rather, the permission checking is done later on through a require statement in another function called in adminAddRelayer function body. Although the final behavior is the same in both cases and the transaction will be reverted if the \textit{msg.sender} is anyone but the admin, there are two considerations: 
\begin{itemize}
    \item The developer has to keep track of two places where there is a revert statement to check the exact same condition making code modifications as well as debugging of the reverted transactions harder.
    \item Reverting an unsuccessful transaction still costs gas for the transaction sender. This means if a transaction is going to be reverted, it should be reverted as quickly as possible which conflicts with what is for adminAddRelayer function.
\end{itemize}

\begin{lstlisting}[language=Solidity, caption=\textit{adminAddRelayer} function from Bridge contract \cite{Chainbridgesolidity2022a}, label={lst:adminAddRelayer}]
function adminAddRelayer(address relayerAddress) external {
    require(
        !hasRole(RELAYER_ROLE, relayerAddress),
        "addr already has relayer role!"
    );
    require(_totalRelayers() < MAX_RELAYERS, "relayers limit reached");
    grantRole(RELAYER_ROLE, relayerAddress);
    emit RelayerAdded(relayerAddress);
}
\end{lstlisting}                        
\textit{revokeRole} function has the same condition as explained above. Both of these functions are modeled with “admin” role in DCR model. This will capture the intended authorization mechanism although it is not directly enforced on \textit{revokeRole} and \textit{adminAddRelayer} functions. 

\subsection{Unclear initial state}
The Bridge contract contains a concept of proposal, and an enum to show the state the proposal is at (listing \ref{lst:proposalstatus}). 

\begin{lstlisting}[language=Solidity, caption=ProposalStatus enum from Chainsafe Bridge contract, label={lst:proposalstatus}]
enum ProposalStatus {
    Inactive,
    Active,
    Passed,
    Executed,
    Cancelled
}
\end{lstlisting}

Implementing states with enums in Solidity helps with ordering of actions. However, the initial state of the contract is unclear. The lack of explicit default initialization is because default value for a Solidity enum is the first item in it. Therefore, the initial proposal state in Bridge contract is \textit{inactive}. Although this is not a weakness, it still makes the implementation less understandable. A proposed and simple solution would be to explicitly initialize the state in the constructor function.


\subsection{Reducible Control-Flow (likewise: Reducible Gas Consumption)}
Listing \ref{lst:reducible} contains a part of \textit{executeProposal} function. The inferred DCR graph from this code snippet in figure \ref{fig:inferredExecuteProposal} shows a call to an external function which decides the rest of control flow. If the call fails and \textit{revertOnFail} variable is set, the rest of the call will just be reverted. In case of it not been set while the external function fails, the outter \textit{executeProposl} function returns with an event emission. The reason for this behavior is two different situations where \textit{executeProposal} is supposed to be called. However, when the developer manually implements \textit{executeProposal} based on its DCR graph (figure \ref{fig:inferredExecuteProposal}), the implementation becomes more intuitive, understandable, and consumes less gas. 
\todo[inline]{Explicitly state the problem, and see if there is a pattern for the problem and possibly automatic detection/patching.}
\todo{Prove your claim based on some sort of complexity measurement!}
\todo{Also prove that it actually uses less gas!}

\begin{lstlisting}[language=Solidity, label={lst:reducible}, caption=Reducible part of executeProposal function from Bridge contract]
proposal._status = ProposalStatus.Executed;
IDepositExecute depositHandler = IDepositExecute(handler);

if (revertOnFail) {
    depositHandler.executeProposal(resourceID, data);
} else {
    try depositHandler.executeProposal(resourceID, data) {} catch (
        bytes memory lowLevelData
    ) {
        proposal._status = ProposalStatus.Passed;
        emit FailedHandlerExecution(lowLevelData);
        return;
    }
}
\end{lstlisting}


\begin{figure}[H]
    \centering
    \includegraphics[width=1\textwidth]{figures/reduced-executeProposl.pdf}
    \caption{Inferred semantics of executeProposal function}
    \label{fig:inferredExecuteProposal}
\end{figure}

\begin{lstlisting}[language=Solidity, label={lst:reduced}, caption=Modified (Reduced) part of executeProposal function from Bridge contract]
IDepositExecute depositHandler = IDepositExecute(handler);

try depositHandler.executeProposal(resourceID, data) {
    proposal._status = ProposalStatus.Executed;
} catch (
    bytes memory lowLevelData
) {
    if (revertOnFail) {
        revert();
    } else {
        emit FailedHandlerExecution(lowLevelData);
        return;
    }
}
\end{lstlisting}

\subsection{Preventing The Nomad Bridge \textit{Mistake}}
Bridging is the practice of connecting two blockchain networks to enable transfer of tokens, information, and functionality between them. Nomad \cite{nomadbridge} is one of these bridging protocols that supports multiple chains.

One of the most recent smart contract hacks happened in August 1st, 2022 on Nomad bridge. Based on the inner workings of bridge smart contracts three specific functions were involved in the flaw that resulted in their vulnerability: \textit{initialize}, \textit{acceptableRoot}, \textit{process}. Without going into much detail, \textit{initialize} function is supposed to correctly initialize \textit{confirmAt} variable that will later be checked inside \textit{acceptableRoot} to allow or disallow processing of a message (using \textit{process} function). The problem arises in \textit{initialize} function by not checking any condition to correctly initialize \textit{confirmAt}, a variable that is later used to authorize the processing of messages. Therefore, the incident in essence is the result of missing a condition before making an event plausible. The condition is now added to their smart contract source code which is available here\footnote{https://github.com/nomad-xyz/monorepo/commit/0e02cc1f09d16f809f5d2d8f05abbeea6d1af04e}. The fundamental problem as demonstrated in figure \ref{fig:nomad} was that \textit{the correct version of check} did not happen in \textit{acceptableRoot} function  (because of a mistake in \textit{initialize}).  

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/nomad-bridge.pdf}
    \caption{Execution condition that was missing in the Nomad bridge hack.}
    \label{fig:nomad}
\end{figure}

While the presented partial model for the condition checking in figure \ref{fig:nomad} seems very trivial, in reality implementing the condition requires two pieces in code to work together (\textit{initialize} and \textit{acceptableRoot}) to perform a correct authorization. The fact that the correct condition can only be checked if the setting of the values is distributed temporally in two code locations adds to the complexity of implementing a correct version.

The compelling aspect of modeling Nomad bridge using DCR graphs is that although it captures the fact that two conditions should align (figure \ref{fig:nomad}) to enable \textit{process} function be called, it is not concerned with the code location this is done. This independency of implementation details not only hides the complexity and lets the modeler visualize the actual intended behavior, but also lets developers using this model have a mind map to follow and check after implementing the contract.  









==> components/patterns.tex <==
\section{Smart Contract Design Patterns}\label{sec:design-patterns}

We categorise all gathered smart contract design patterns that are related to the business process of the contract into the following categories:
\begin{enumerate}
    \item \textbf{Pure time-based constraints}: Time-based patterns imply constraints about the timing of activities. They define deadlines, delays, and adaptive behaviour for them.
    \item \textbf{Roles and access control}: Role-based access control~\cite{sandhu1998role} restricts access to given functions to predefined roles.
    \item \textbf{Action dependencies and contract staging}: A business process may impose an order on any pair of activities.
    \item \textbf{Structural patterns}: These impose a certain structure on the contract business process (and the implementation as a result). These patterns are created by combining other design patterns. 
\end{enumerate}
Note that many patterns combine aspects of two of the above-mentioned categories; Fig.~\ref{fig:states-ordering} depicts a classification of 20 design patterns we have identified. We elucidate these patterns further below.

\begin{figure}[t]
    \centering
    \includegraphics[scale=.7]{figures/venn-diagram.drawio.pdf}
    \caption{Classification of smart contract design patterns with respect to their underlying business processes and the overlap between classes}
    \label{fig:states-ordering}
\end{figure}
\subsection{Time Constraint}\label{sec:time-constraint}
In some cases, a business process has multiple stages of execution.
An implementation needs to ensure that code execution adheres to these stages.
This stage-based execution can be strictly time-based or based on
action dependencies. If this stage-based execution is solely based
on a certain time having elapsed, we call it time constraint \cite{EmpiricalAnalysisSmart2017}. The simplest form of this pattern\footnote{https://github.com/mojtaba-eshghie/SolidityDesignPatternsDCRGraph/\#time-constrained} is used
in the lottery contract source code \cite{lotteryContract}; here, the
\emph{payoutReady} function reverts the transaction if it is not ready yet.

%\begin{lstlisting}[language=Solidity, label={lst:time-constraint-simple}, caption=Simple example of time constraint pattern used in lottery smart contract]
%function payoutReady() constant returns %(bool) {
%    return decidingBlock <= btcRelay.getLastBlockHeight();
%}
%function processPayout() returns (bool %done) {
%    if (!payoutReady()) throw;
%    ...
%}
%\end{lstlisting}
More complex time constraints enable or disable parts of a function based on a certain time or stage of the execution; i.\,e., the success of a function call depends on the time (block number) or contract state.
A prominent example of such time-constraint is the ChainSafe bridge Solidity contract~\cite{Chainbridgesolidity2022a}. In this contract, the function \emph{voteProposal} has multiple \emph{require} statements that control action dependencies and cause the same function to have different results based on the time of calling and what actions were carried out so far in the contract's lifetime.
%Furthermore, a more obvious example of time constraint is where the expiration block of a \emph{proposal} is checked after all the action dependencies are ensured.

\subsection{Time Incentivisation}\label{sec:time-incent}
In Ethereum, smart contract code execution works as a reactive system.
Transactions are executed by specific function calls.
There are scenarios where certain actions have to be performed at a specific time or when a specific condition is fulfilled. One example of such a scenario is a game smart contract where each user should roll the dice so that the game can continue. A user may decide to leave the game without it. This lack of action may prevent a process from progressing and may incentivize adversarial interests.

It is not possible to implement a scheduling system without an external oracle such as Chainlink cron jobs~\cite{SolidityCronJobs}. However, these require an \emph{oracle}, which incorporates off-chain information on a smart contract (see \P\ref{sec:oracle}). This greatly increases the complexity of a smart contract.

Instead, the \emph{time incentivisation} pattern can
motivate parties to cooperate even in the existence of conflicting interests.
In the game contract example, an incentivisation stipulates a deadline at which an actor has to make a move. An actor that misses the deadline is punished, while other players are rewarded, for example, by forfeiting the bets of tardy actors.
This pattern is also used and modeled in the Casino contract (see \P\ref{sec:casino}).

\subsection{Automatic deprecation}
Automatic deprecation is the opposite of a time constraint (based on the time period at which an activity is executable). It stipulates a deprecation time (block number) after which a function is not executable anymore \cite{DesignPatterns2018}. 

\subsection{Rate limiting}\label{sec:rate-limiting}
Rate limiting imposes a limit on the number of successful function calls by a participating user during a specific time period \cite{RateLimitingEthereum}. The time period typically starts when the contract is deployed. At each request, it is checked whether the request is within the limits of the total amount of assets that can be withdrawn (or the number of any sensitive actions). In Figure \ref{fig:rate-limiting-timeline}, the first and second requests are successful since the total does not exceed the limit of the period. However, the third request fails (reverts) because of the limit being violated by the transaction. Furthermore, the last transaction succeeds because the period is renewed, and \emph{total} is initialized to zero for the new period.

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.8]{figures/rate-limiting.pdf}
    \caption{Rate limiting pattern in action}
    \label{fig:rate-limiting-timeline}
\end{figure}

\subsection{Timed Temporal Constraint (Speed Bump)}\label{sec:speed-bump}
A \emph{speed bump} is used to slow down critical operations such as the withdrawal of assets, authorization of significant actions, etc. \cite{SpeedBumpsEthereum}. It puts a temporal barrier that gives enough time to automatic or manual monitoring systems to detect a problematic activity and mitigate it. This pattern is a generalized version of the time constraint pattern where the participating user can only execute an action
after a predefined time period has passed (see Fig.~\ref{fig:speed-bump-timeline}). The constrained action in this figure is \emph{withdraw}. Withdrawing from the contract is only possible via registering the request in one transaction, waiting for a predefined period, and then, sending the actual withdraw request. Any withdraw transaction before the end of the waiting period will be reverted (in the red time window in Fig.~\ref{fig:speed-bump-timeline}).


\begin{figure}[t]
    \centering
    \includegraphics[scale=0.8]{figures/speed-bump.pdf}
    \caption{Timed temporal constraint design pattern in action.}
    \label{fig:speed-bump-timeline}
\end{figure}


\subsection{Safe Self-Destruction}\label{sec:safe-self-destruction}
It is possible to define a function in Solidity that uses \emph{selfdestruct(address target)} to destroy the contract intentionally and send all Ether in the contract account to the target. Safe self-destruction 
%concerns ensuring that execution of this function is limited to only 
is about limiting the execution of the function to
specific roles such as the administrator or contract deployer \cite{DesignPatterns2018, EmpiricalAnalysisSmart2017}.

\subsection{Access Control}\label{sec:access-control}
Access control restricts access to desired functions to only a subset of accounts calling them \cite{EmpiricalAnalysisSmart2017,DesignPatterns2018,SolidityPatternsWebsite}. One typical implementation of this pattern in smart contracts is to initialize a variable \emph{owner} to the contract deployer, and only let this account make transactions to desired functions successfully.

\subsection{Commit and reveal}\label{sec:commit-and-reveal}
This pattern builds contracts that work in two phases. Phase 1 is submitting a result, bidding, etc.; Phase 2 is checking and revealing the submitted values. In a public permissionless blockchain platform such as Ethereum, transaction data is public \cite{DesignPatterns2018}. Therefore, if a transaction sends a secret in plain text, participants in the blockchain consensus protocol can see the plain text value even before the transaction is appended to the end of the block. This means an attacker can overhear the unappended secret, create its own high-priority transaction based on that secret, and submit it to be appended to the blockchain. This attack is often referred to as \emph{front-running}. To mitigate the effects of this attack, data that is subject to front-running should be used in two phases: first, committing to the secret by sending the hash, and second, revealing the secret after either all parties have committed, or the committed period is over.  

\subsection{Circuit breaker (Emergency Stop)}\label{sec:circuit-breaker}
Smart contracts run autonomously on the blockchain platform, and there is no inherent option provided by the platform to stop their lifecycle without programming that into the smart contract code itself. This pattern is used to stop all normal functionality of the smart contracts until a manual/automatic investigation is performed by the smart contract owner account \cite{securityPatterns}. This pattern can be triggered by other contract functions following patterns such as a timed temporal constraint (\P\ref{sec:speed-bump}). 

\subsection{Escapability}\label{sec:escapable}
There have been cases where a vulnerability in the contract triggered by a certain transaction can lead to all the funds being locked in the smart contract. In situations like this, the logic of the smart contract prevents the funds from being withdrawn. One popular such lock-in incident happened in 2022 with Akutars NFT \cite{ExplainedAkutarsNFT} at which millions of dollar worth of Ether were locked inside the contract.

To mitigate the harm of such vulnerabilities, a smart contract can contain a function whose logic is independent on the main contract logic; when triggered, it can potentially disable all or a subset of functions and withdraw all assets in the contract to a certain address. This new address can be the upgraded version of the contract that contains a patch for the vulnerability. 


\subsection{Checks, Effects, Interactions}\label{sec:checks-effects-interactions}
As the name suggests, this pattern is concerned with the order of certain activities, especially when interactions with other contracts (external calls) happen \cite{securityPatterns,SolidityPatternsWebsite}. External calls can be risky as the call target is untrusted. The risks are two-fold: (1) the target of the call can sometimes execute code in the context of the caller contract, or (2) call into the same caller function again and abuse the logic (e.\,g., reentrancy~\cite{dynamicVul}). To prevent such exploits, before making an external call (\emph{interaction}), the caller first performs \emph{checks} on its bookkeeping variables\footnote{Variables keeping the balance of tokens, assets, etc.}. Then, it modifies these bookkeeping variables based on the business logic \emph{(effects)}. Lastly, there will be \emph{interactions} with other contract functions or external calls to other contracts.

\subsection{Mutex}\label{sec:mutex}
This pattern prevents accessing a resource twice in the same transaction. By obtaining and releasing a lock prior to and after executing the contract function \cite{securityPatterns}, it mainly prevents the same class of vulnerabilities and flaws \P \ref{sec:checks-effects-interactions} prevents. Therefore, while the lock is not released it is not possible to reenter the same function (call it again) during the same transaction. 

\subsection{Guard Check}\label{sec:guard-check}
A guard check validates user inputs, and performs checks on bookkeeping variables and invariants before the execution of the function body (mainly as a \emph{require} statement) \cite{hodlit}. This pattern is often applied using function \emph{modifiers}.

\subsection{Abstract Contract States}\label{sec:fsm}
In most real-world processes that underlie a smart contract,
there is an action dependency that imposes a partial order on action executions.
The smart contract has to adhere to this order, as shown in detail in the casino contract (\P\ref{sec:casino}). The abstract contract states is a design pattern that uses Solidity \emph{enum} to create a finite state automaton \cite{DesignPatterns2018}. The state transitions of this FSA modify the set of executable functions, establishing a partial order among action executions.


\subsection{Secure Ether Transfer}\label{sec:secure-ether-transfer}
This structural design pattern imposes a design choice between various ways of sending ether from a contract to another contract (\emph{send}, \emph{transfer}, and \emph{call}) \cite{SolidityPatternsWebsite}. Using each of them requires a distinct way of ensuring the target contract cannot harm the contract sending Ether. One central design choice in this pattern involves whether or not to let the contract receiving Ether execute extra bookkeeping operations. The bookkeeping operations consume more gas, especially since they involve modifying Ethereum \emph{storage}. Gas is the cost the transaction sender pays to blockchain miners to include its transaction. 
Based on the specific design choice, secure ether transfer is often accompanied by a mutex and guard check (\P \ref{sec:mutex} and \P \ref{sec:guard-check}) design patterns. 



\subsection{Oracle}\label{sec:oracle}
Oracles enable smart contracts to incorporate off-chain data in their execution and push information from a blockchain to external systems \cite{EmpiricalAnalysisSmart2017,DesignPatterns2018}. Without the involvement of oracles, blockchain systems lose their determinism because of a lack of consensus between different nodes executing smart contracts that read data from variable off-chain sources. To further avoid indeterminism when querying an oracle, multiple data sources are used whenever possible. This is to form a quorum of responders to the same query.

This design pattern employs an external call to another \emph{service smart contract} (data source) to register the request for off-chain data. This registration call information should also be kept in bookkeeping variables inside the contract itself. When the data is ready in the service contract, it will inform the main contract about the result by calling a specific \emph{callback} function.

\subsection{Token Design Patterns}\label{sec:token-design-patterns}
Tokens represent assets, their behavior, and manageability \cite{EmpiricalAnalysisSmart2017}. Ethereum smart contracts enable developers to build tokens according to their requirements. Token standards (such as ERC-20, ERC-721, and ERC-777) define an interface that the token contract should expose to be composable with other contracts. 

\subsection{Pull Over Push}\label{sec:pull-over-push}
A contract might need to send a token or Ether to one or more accounts. The ``pull over push'' pattern discourages pushing tokens or Ether to the destination. Rather, it encourages exposing a \emph{withdraw} function that those specific accounts can call \cite{DesignPatterns2018}. This inclination towards pull is based on the fact that when sending Ether or tokens via any external call (even when adhering to patterns such as \P \ref{sec:secure-ether-transfer}), the called function in the target might act in an unexpected manner.  


\subsection{Upgradability}\label{sec:upgradability}
The upgradability design pattern consists of several contracts that enable easy upgrading of immutable smart contracts \cite{designPatternsGas,DesignPatterns2018, }. This design pattern consists of up to five subpatterns, which we do not classify as stand-alone patterns here.
(1) The proxy subpattern involves a contract that holds the addresses of referred smart contracts in its state variables. This allows updating contracts without updating all smart contracts that directly call the old contract. (2) The data segregation subpattern separates the logic and data layers by storing data in a separate smart contract, reducing the cost of data migration when code functionality changes. (3) The satellite pattern outsources functional units to separate satellite contracts and stores their addresses in a base contract. This allows easy modification and replacement of contract functionality. (4) In another subpattern, the register contract tracks different versions of a contract and points to the latest one, which participants must query before interacting. (5) The relay pattern uses a proxy contract to forward calls and data to the newest contract version while keeping the old contract address. In conclusion, these subpatterns provide flexibility in upgrading smart contracts, reduce updating costs, and promote separation of concerns, making contracts more modular and manageable~\cite{DesignPatterns2018}.

\subsection{Governance}\label{sec:governance}
On-chain governance is a crucial component of decentralised protocols, allowing for decision-making on parameter changes, upgrades, and management \cite{governanceLiteratureReview, EmpiricalAnalysisSmart2017}. A popular example of on-chain governance is the Compound protocol \cite{CompoundV2Docs}. The upgrade functionality (\P \ref{sec:upgradability}) is the most powerful feature of the governance design pattern, enabling governance to change almost everything, including the governance mechanism itself.

The governance mechanism in the Compound permits COMP token holders to engage in decision-making. This pattern is composed of various smart contracts, with the governance contract at its core serving as the overseer for other contracts in the protocol. The governance contract is permissioned to handle a range of functions, including implementing new markets, modifying parameters, and upgrading contracts. When a proposal is submitted, all COMP token holders are eligible to cast a vote, with each token counting as a single vote. A proposal is approved if it receives a majority of votes in favor, and if at least 4\% of the total supply of COMP participates in voting. After a proposal is approved, the protocol's smart contracts automatically execute the proposal. 

